Beyond the Bridge: Contention-Based Covert and Side Channel Attacks on Multi-GPU Interconnect

High-speed interconnects, such as NVLink, are integral to modern multi-GPU systems, acting as a vital link between CPUs and GPUs. This study highlights the vulnerability of multi-GPU systems to covert and side channel attacks due to congestion on interconnects. An adversary can infer private information about a victim's activities by monitoring NVLink congestion without needing special permissions. Leveraging this insight, we develop a covert channel attack across two GPUs with a bandwidth of 45.5 kbps and a low error rate, and introduce a side channel attack enabling attackers to fingerprint applications through the shared NVLink interconnect.

==> attakmodel.tex <==
\section{Threat Model}
\label{sec:threatmodel}


\yicheng{Need one figure for threat model}

==> mitigation.tex <==
\section{Mitigation} 
\label{sec:mitigation}

==> relatedwork.tex <==
\section{Related Work}

Several works have been focused on security aspects of multi-GPU systems. Dutta et al. ~\cite{dutta2023spy} has shown the possibility of contention-based micro-architectural attacks in multi-GPU systems utilizing L2 cache.   

\noindent \textbf{{Microarchitectural attacks on GPUs}} 

\noindent \textbf{{Other interconnect congestion side-channel.}} 
